X-ray bright active galactic nuclei in massive galaxy clusters III: New insights into the triggering mechanisms of cluster AGN

We present the results of a new analysis of the X-ray selected Active Galactic Nuclei (AGN) population in the vicinity of 135 of the most massive galaxy clusters in the redshift range of 0.2 < z < 0.9 observed with Chandra. With a sample of more than 11,000 X-ray point sources, we are able to measure, for the first time, evidence for evolution in the cluster AGN population beyond the expected evolution of field AGN. Our analysis shows that overall number density of cluster AGN scales with the cluster mass as $\sim M_{500}^{-1.2}$. There is no evidence for the overall number density of cluster member X-ray AGN depending on the cluster redshift in a manner different than field AGN, nor there is any evidence that the spatial distribution of cluster AGN (given in units of the cluster overdensity radius r_500) strongly depends on the cluster mass or redshift. The $M^{-1.2 \pm 0.7}$ scaling relation we measure is consistent with theoretical predictions of the galaxy merger rate in clusters, which is expected to scale with the cluster velocity dispersion, $\sigma$, as $ \sim \sigma^{-3}$ or $\sim M^{-1}$. This consistency suggests that AGN in clusters may be predominantly triggered by galaxy mergers, a result that is further corroborated by visual inspection of Hubble images for 23 spectroscopically confirmed cluster member AGN in our sample. A merger-driven scenario for the triggering of X-ray AGN is not strongly favored by studies of field galaxies, however, suggesting that different mechanisms may be primarily responsible for the triggering of cluster and field X-ray AGN.

==> TestHubble.tex <==

\section{Preliminary Spectral Identification and Visual Classification of Cluster Member AGN}


We have carried out a preliminary attempt to confirm cluster member AGN spectroscopically by searching the NASA/IPAC Extragalactic Database (NED) for optical spectroscopic counterparts for our X-ray point source positions. The search circle around each X-ray source is $2 \arcsec$, sufficiently large to account for the expected positional uncertainties on our X-ray sources. Control tests that added random offsets to the X-ray source positions suggest that our expected number of ``false positives'' (i.e. finding a spectroscopic counterpart at the cluster redshift by chance coincidence) is negligible. Where we find a spectroscopic counterpart to the X-ray source with a redshift $\mysub{z}{cp}$ satisfying $c\vert \mysub{z}{cluster}-\mysub{z}{cp} \vert < 5000 \km \s^{-1}$, we identify that X-ray source to be a spectroscopically confirmed cluster member. In total, we find that 88 of our X-ray AGN have spectroscopic counterparts within $2\arcsec$ of the source position. 


We then searched the {\it Hubble} archive for images at each of these source positions made with either the ACS or WFC3 cameras. The {\it Hubble} images were registered to the \cha \ images and cleaned of cosmic rays using the Laplacian edge detection algorithm of \cite{VanDokkum2001}. After these steps, 23 of the X-ray AGN had {\it Hubble} images deemed suitable for a preliminary visual classification of their morphologies. 

Source catalogs for each {\it Hubble} field were produced using \sext \ \citep{Bertin1996} in a single filter. For each X-ray AGN we selected three control galaxies with similar optical magnitudes and clustercentric distances to the X-ray AGN. We then produced postage stamp images of the 5$\arcsec$ radius surrounding each galaxy in both the AGN and control sample, utilizing up to three filters of imaging data for each galaxy when available. The postage stamp {\it Hubble} images for all 23 X-ray AGN can be found in Figure \ref{XRaySourceImages}. Information about the filters and source positions are given in Table \ref{XRaySourceTab}. 



\begin{table*}
\caption{\label{XRaySourceTab}  Information about the {\it Hubble} images for all 23 spectroscopically confirmed X-ray AGN. For each source position, we denote the filters used for the images presented in Figure \ref{XRaySourceImages}. }
\centering

\begin{tabular}{ c c c c c  }\\
  \hline 
RA & DEC & Filter 1 & Filter 2  & Filter 3   \\ 
\hline\hline


3.53939 & -30.41137 &  F606W &  &  \\ 
3.55994 & -30.37781 &  F606W &  &  \\ 
3.61061 & -30.39563 &  F606W &  &  \\ 
4.63350 & 16.49064 &  F606W &  &  \\ 
4.65420 & 16.46027 &  F775W & F606W & F555W \\ 
6.38361 & -12.38467 &  F555W &  &  \\ 
28.16550 & -13.92369 &  F775W & F625W &  \\ 
28.28761 & -13.96692 &  CLEAR1L &  &  \\ 
28.30403 & -13.89717 &  F606W &  &  \\ 
29.99430 & -8.82704 &  F606W &  &  \\ 
73.50511 & 2.96277 &  F606W &  &  \\ 
73.55489 & 2.95945 &  F606W &  &  \\ 
139.43829 & 51.71885 &  CLEAR1L &  &  \\ 
146.80429 & 76.38735 &  F125W & F110W & F606W \\ 
151.72157 & 32.00314 &  F606W &  &  \\ 
177.39105 & 22.37405 &  F775W & F606W & F475W \\ 
181.55492 & -8.79565 &  F775W & F606W & F475W \\ 
186.71535 & 21.87390 &  F606W &  &  \\ 
186.75880 & 33.56825 &  F775W & F625W &  \\ 
212.63080 & 52.25929 &  F775W &  &  \\ 
224.31136 & 22.32598 &  F850LP & F775W &  \\ 
243.90677 & -6.18664 &  F606W &  &  \\ 
328.38098 & 17.69271 &  F125W & F850LP &  \\ 
\hline\hline

\end{tabular}
\end{table*}





Galaxy morphologies were determined visually to fall into one of the following classes: 1) {\bf Disturbed} galaxies which have clear signatures of disruptions from mergers such as tidal tails; 2) {\bf Undisturbed}  galaxies with no apparent disruptions; 3) Nearby {\bf Neighbor} galaxies which, while not having evidence for major disruptions, are sufficiently near to other galaxies to suggest an imminent merger; 4) {\bf Stellar} galaxies whose morphologies could not be distinguished from a point source; or 5) {\bf Empty} images where the host of the X-ray point source could not be determined. All of the co-authors except authors SE, RC, and AvdL did the morphology classification on all 92 galaxies. None of the participating co-authors knew which of the galaxies were the hosts of the X-ray AGN and which were control galaxies in advance. We then determined the fraction of galaxies within each of these morphological classes for both the normal galaxies and X-ray AGN. 


Our main finding is that galaxies hosting X-ray AGN were classified as {\bf Disturbed} at higher rates than the control sample. The {\bf Disturbed} vote fractions for the X-ray AGN and control sample are $22\% $ (30/138) and $10\% $ (43/414), respectively. We utilize a two-sided Student's t-test to determine the probability of these two measurements arising from the same underlying population. Assuming a null hypothesis where the X-ray AGN and control samples have the same average fractions of disturbed galaxies, then we have a probability of $p=0.043$ of measuring a larger absolute difference in the disturbed fractions of the two samples.\footnote{This particular $p$ value assumes equal variance for the X-ray AGN and control samples. If we don't assume equal variance, then the probability of measuring a larger absolute difference in the means increases to $p=0.097$.} Galaxies hosting X-ray AGN were equally likely to be classified as {\bf Neighbor, Empty, Stellar}, and {\bf Undisturbed} as their control galaxies. Applying a simple weighting scheme that weights more strongly sources where all voters agree on a particular classification leads to similar results. In conclusion, while there is some initial evidence that X-ray AGN in clusters may be preferentially hosted in galaxies with disturbed morphologies (consistent with a merger driven scenario), larger data samples and more robust (preferably automated) classification schemes will be required to further investigate the extent to which mergers may be responsible for the triggering of X-ray AGN in galaxy clusters.  

One particular galaxy of note identified in this study is the X-ray AGN at $\rm{RA (J2000)}= 04^{h} 54^{m} 13.17^{s}$, $ \rm{DEC (J2000)}=+02^{\circ} 57^{m} 34.0^{s}$ in the galaxy cluster Abell 520, a cluster galaxy which hosts a clear partial Einstein ring that has not yet been published in the literature.    



% \begin{table*}
% \small
% \caption{\label{XRayClassTab} The morphological classifications for the 23 spectroscopically confirmed cluster member X-ray AGN with {\it Hubble} imaging. The columns denote: 1) the right ascension of the AGN as determined by \cha, in J2000; 2) the declination of the AGN in J2000; 3) the number of classifiers that determined this galaxy as {\bf Disturbed}; 4) the number of classifiers that determined this galaxy as {\bf Neighbor}; 5) the number of classifiers that determined this galaxy as {\bf Undisturbed}; 6) the number of classifiers that determined this galaxy as {\bf Star}; and 7) the number of classifiers that determined this galaxy as {\bf Empty}. The final three rows present the statistics for these classification results: the first two rows show the distribution of votes in each category as measured for all 23 AGN, along with the $95\%$ confidence interval on the fraction as determined by the appropriate $\beta$-distribution for the numerator and denominator. The last row shows the values of the weighted averages for each morphological class alongside two times the variance ($2\sigma$) about that average given the sample, which corresponds to our best estimate for the $95\%$ confidence interval for the weighted average.        }
% \centering

% \begin{tabular}{ c c c c c c c }\\

% \hline 

% RA & DEC & Disturbed & Neighbor & Undisturbed & Star & Empty   \\ 
% \hline\hline
 
% 00 14 14.39 & $-$30 22 40.12 & 6 & 0 & 0 & 0 & 0  \\
% 00 14 26.55 & $-$30 23 44.27 & 4 & 0 & 2 & 0 & 0  \\
% 00 14 09.45 & $-$30 24 40.93 & 0 & 0 & 6 & 0 & 0  \\
% 00 18 32.04 & 16 29 26.30 & 0 & 0 & 0 & 6 & 0  \\
% 00 18 37.01 & 16 27 36.97 & 0 & 5 & 1 & 0 & 0  \\
% 00 25 32.07 & $-$12 23 04.81 & 0 & 1 & 5 & 0 & 0  \\
% 01 52 39.72 & $-$13 55 25.28 & 0 & 3 & 2 & 0 & 1  \\
% 01 53 12.97 & $-$13 53 49.81 & 4 & 1 & 1 & 0 & 0  \\
% 01 53 09.03 & $-$13 58 00.91 & 3 & 3 & 0 & 0 & 0  \\
% 01 59 58.63 & $-$08 49 37.34 & 2 & 0 & 4 & 0 & 0  \\
% 04 54 01.23 & 02 57 45.97 & 0 & 3 & 3 & 0 & 0  \\
% 04 54 13.17 & 02 57 34.02 & 0 & 0 & 6 & 0 & 0  \\
% 09 17 45.19 & 51 43 07.86 & 0 & 0 & 4 & 2 & 0  \\
% 09 47 13.03 & 76 23 14.46 & 1 & 3 & 2 & 0 & 0  \\
% 10 06 53.18 & 32 00 11.30 & 0 & 6 & 0 & 0 & 0  \\
% 11 49 33.85 & 22 22 26.58 & 0 & 0 & 1 & 5 & 0  \\
% 12 06 13.18 & $-$08 47 44.34 & 0 & 0 & 6 & 0 & 0  \\
% 12 26 51.68 & 21 52 26.04 & 1 & 0 & 5 & 0 & 0  \\
% 12 27 02.11 & 33 34 05.70 & 2 & 1 & 2 & 0 & 1  \\
% 14 10 31.39 & 52 15 33.44 & 4 & 0 & 2 & 0 & 0  \\
% 14 57 14.73 & 22 19 33.53 & 0 & 0 & 6 & 0 & 0  \\
% 16 15 37.62 & $-$06 11 11.90 & 2 & 0 & 4 & 0 & 0  \\
% 21 53 31.44 & 17 41 33.76 & 1 & 0 & 5 & 0 & 0  \\



% \hline\hline
% Total Votes ( 138 )&   & 30 & 26 & 67 &  13 & 2 \\
% Vote Fractions (\%) &  & $22^{+7}_{-6}$ & $19^{+7}_{-6}$ & $49^{+7}_{-9}$ & $9^{+6}_{-4}$ & $1 ^{+4}_{-1}$ \\ 
% Weighted Averages (x 100) & & $21 \pm 14$ & $19 \pm 13$ & $49 \pm 17$ & $9 \pm 12$ &  $ 0.7 \pm 1$\\









% \hline\hline

% \end{tabular}
% \end{table*}




% \begin{table*}
% \small

% \caption{\label{GalClassTab} The morphological classifications for the 69 control galaxies to the X-ray AGN. The columns denote: 1) the right ascension of the AGN as determined by \cha, in J2000; 2) the declination of the AGN in J2000; 3) the number of classifiers that determined this galaxy as {\bf Disturbed}; 4) the number of classifiers that determined this galaxy as {\bf Neighbor}; 5) the number of classifiers that determined this galaxy as {\bf Undisturbed}; 6) the number of classifiers that determined this galaxy as {\bf Star}; and 7) the number of classifiers that determined this galaxy as {\bf Empty}. 
% The final three rows present the statistics for these classification results: the first two rows show the distribution of votes in each category as measured for all 23 AGN, along with the $95\%$ confidence interval on the fraction as determined by the appropriate $\beta$-distribution for the numerator and denominator. The last row shows the values of the weighted averages for each morphological class alongside two times the variance ($2\sigma$) about that average given the sample, which corresponds to our best estimate for the $95\%$ confidence interval for the weighted average.     }
% \centering

% \begin{tabular}{ c c c c c c c }\\
%   \hline 
% RA & DEC & Disturbed & Neighbor & Undisturbed & Star & Empty   \\ 
% \hline\hline


% 00 14 16.63 & $-$30 23 03.48 & 4 & 0 & 1 & 0 & 1  \\
% 00 14 18.58 & $-$30 21 25.56 & 0 & 2 & 4 & 0 & 0  \\
% 00 14 18.79 & $-$30 23 13.56 & 1 & 5 & 0 & 0 & 0  \\
% 00 14 18.91 & $-$30 23 49.92 & 0 & 6 & 0 & 0 & 0  \\
% 00 14 19.30 & $-$30 23 31.92 & 0 & 1 & 5 & 0 & 0  \\
% 00 14 21.10 & $-$30 24 03.24 & 0 & 2 & 4 & 0 & 0  \\
% 00 14 21.29 & $-$30 23 45.96 & 0 & 2 & 4 & 0 & 0  \\
% 00 14 22.73 & $-$30 23 49.92 & 3 & 0 & 3 & 0 & 0  \\
% 00 14 27.00 & $-$30 23 34.80 & 0 & 1 & 5 & 0 & 0  \\
% 00 18 25.42 & 16 28 09.48 & 2 & 1 & 3 & 0 & 0  \\
% 00 18 29.42 & 16 28 19.20 & 1 & 1 & 4 & 0 & 0  \\
% 00 18 29.98 & 16 28 51.24 & 0 & 0 & 6 & 0 & 0  \\
% 00 18 30.94 & 16 25 48.00 & 0 & 5 & 0 & 0 & 1  \\
% 00 18 35.30 & 16 25 48.36 & 0 & 2 & 3 & 0 & 1  \\
% 00 18 36.53 & 16 27 17.28 & 1 & 4 & 0 & 0 & 1  \\
% 00 25 24.67 & $-$12 22 29.28 & 0 & 4 & 2 & 0 & 0  \\
% 00 25 26.83 & $-$12 22 28.56 & 0 & 3 & 3 & 0 & 0  \\
% 00 25 34.08 & $-$12 23 14.64 & 5 & 0 & 0 & 0 & 1  \\
% 01 52 38.90 & $-$13 54 56.16 & 0 & 3 & 3 & 0 & 0  \\
% 01 52 38.93 & $-$13 55 13.08 & 0 & 5 & 0 & 1 & 0  \\
% 01 52 42.29 & $-$13 56 39.12 & 0 & 4 & 2 & 0 & 0  \\
% 01 53 13.06 & $-$13 56 40.56 & 0 & 1 & 4 & 0 & 1  \\
% 01 53 16.22 & $-$13 52 18.84 & 0 & 3 & 3 & 0 & 0  \\
% 01 53 18.10 & $-$13 57 38.52 & 0 & 5 & 1 & 0 & 0  \\
% 01 53 18.70 & $-$13 57 11.88 & 2 & 4 & 0 & 0 & 0  \\
% 01 53 20.30 & $-$13 53 26.16 & 2 & 0 & 4 & 0 & 0  \\



% \hline\hline

% \end{tabular}
% \end{table*}

% \addtocounter{table}{-1}

% \begin{table*}

% \small
% \caption{\label{GalClassTab} Continued       }
% \centering

% \begin{tabular}{ c c c c c c c }\\
%   \hline 
% RA & DEC & Disturbed & Neighbor & Undisturbed & Star & Empty   \\ 
% \hline\hline


% 01 59 48.41 & $-$08 50 37.68 & 0 & 2 & 4 & 0 & 0  \\
% 01 59 52.82 & $-$08 48 55.08 & 1 & 1 & 4 & 0 & 0  \\
% 01 59 54.00 & $-$08 49 41.52 & 4 & 2 & 0 & 0 & 0  \\
% 04 54 13.25 & 02 57 4.68 & 0 & 1 & 5 & 0 & 0  \\
% 04 54 15.94 & 02 58 18.84 & 1 & 2 & 3 & 0 & 0  \\
% 04 54 20.59 & 02 56 41.28 & 0 & 0 & 6 & 0 & 0  \\
% 04 54 03.19 & 02 56 4.20 & 0 & 0 & 6 & 0 & 0  \\
% 04 54 03.41 & 02 55 40.80 & 0 & 0 & 6 & 0 & 0  \\
% 04 54 05.98 & 02 55 54.84 & 0 & 0 & 6 & 0 & 0  \\
% 09 17 50.64 & 51 43 27.48 & 0 & 0 & 5 & 1 & 0  \\
% 09 17 51.12 & 51 43 17.40 & 0 & 0 & 6 & 0 & 0  \\
% 09 17 51.77 & 51 42 57.24 & 0 & 1 & 4 & 1 & 0  \\
% 09 47 00.91 & 76 23 13.56 & 0 & 0 & 6 & 0 & 0  \\
% 09 47 26.02 & 76 23 24.72 & 0 & 0 & 6 & 0 & 0  \\
% 09 47 28.03 & 76 22 49.08 & 0 & 0 & 4 & 2 & 0  \\
% 10 06 49.87 & 32 01 27.84 & 0 & 4 & 2 & 0 & 0  \\
% 10 06 55.68 & 32 01 11.28 & 1 & 3 & 2 & 0 & 0  \\
% 10 06 57.96 & 32 01 13.08 & 0 & 1 & 5 & 0 & 0  \\
% 11 49 32.95 & 22 23 40.92 & 0 & 2 & 4 & 0 & 0  \\
% 11 49 40.20 & 22 22 59.88 & 0 & 0 & 6 & 0 & 0  \\
% 11 49 40.46 & 22 23 22.20 & 0 & 0 & 6 & 0 & 0  \\
% 12 06 11.74 & $-$08 47 54.24 & 0 & 1 & 5 & 0 & 0  \\
% 12 06 13.10 & $-$08 46 43.32 & 3 & 0 & 3 & 0 & 0  \\
% 12 06 06.96 & $-$08 48 12.96 & 1 & 1 & 4 & 0 & 0  \\
% 12 26 48.86 & 21 53 17.16 & 0 & 4 & 2 & 0 & 0  \\
% 12 26 51.98 & 33 32 51.00 & 3 & 0 & 0 & 0 & 3  \\
% 12 26 52.54 & 21 51 34.56 & 0 & 1 & 5 & 0 & 0  \\
% 12 26 52.92 & 21 52 32.52 & 0 & 1 & 5 & 0 & 0  \\
% 12 26 55.75 & 33 32 11.40 & 0 & 2 & 4 & 0 & 0  \\
% 12 27 04.01 & 33 33 07.56 & 3 & 0 & 2 & 0 & 1  \\



% \hline\hline

% \end{tabular}
% \end{table*}

% \addtocounter{table}{-1}


% \begin{table*}
% \small

% \caption{\label{GalClassTab}  Continued      }
% \centering

% \begin{tabular}{ c c c c c c c }\\
%   \hline 
% RA & DEC & Disturbed & Neighbor & Undisturbed & Star & Empty   \\ 
% \hline\hline


% 14 10 22.32 & 52 17 45.96 & 0 & 4 & 1 & 0 & 1  \\
% 14 10 30.53 & 52 16 59.52 & 1 & 1 & 1 & 0 & 3  \\
% 14 10 33.10 & 52 17 54.24 & 0 & 1 & 5 & 0 & 0  \\
% 14 57 11.59 & 22 19 58.44 & 0 & 1 & 5 & 0 & 0  \\
% 14 57 12.12 & 22 19 50.88 & 0 & 2 & 4 & 0 & 0  \\
% 14 57 12.67 & 22 21 4.68 & 0 & 0 & 6 & 0 & 0  \\
% 16 15 36.43 & $-$06 09 45.00 & 0 & 3 & 3 & 0 & 0  \\
% 16 15 37.42 & $-$06 10 36.12 & 0 & 1 & 1 & 2 & 2  \\
% 16 15 42.43 & $-$06 10 34.68 & 0 & 1 & 5 & 0 & 0  \\
% 21 53 31.08 & 17 41 24.72 & 0 & 1 & 5 & 0 & 0  \\
% 21 53 33.48 & 17 41 57.84 & 0 & 0 & 6 & 0 & 0  \\
% 21 53 33.98 & 17 41 14.28 & 4 & 2 & 0 & 0 & 0  \\


% \hline\hline
% Total Votes ( 414 ) &   & 43 & 110 & 232 &  7 & 22 \\
% Vote Fractions (\%) &  & $10^{+4}_{-2}$ & $27^{+4}_{-4}$ & $56^{+4}_{-5}$ & $2^{+1}_{-2}$ & $5 ^{+3}_{-2}$ \\ 
% Weighted Averages (x 100) & & $10 \pm 6$ & $24 \pm 8$ & $61 \pm 9$ & $1 \pm 1$ &  $ 4 \pm 4$\\

% \hline\hline

% \end{tabular}
% \end{table*}






\clearpage




 \begin{figure*}
 \centering

\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{3_53939_-30_41137_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{3_55994_-30_37781_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{3_61061_-30_39563_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{4_63350_16_49064_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{4_65420_16_46027_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{6_38361_-12_38467_HubbleImage.jpg}





\caption{\label{XRaySourceImages}  The 23 spectroscopically confirmed X-ray images in our sample with follow-up {\it Hubble} imaging. The cross in each image denotes the position of the X-ray source, and the dashed circle corresponds to a radius of 2\arcsec \ surrounding the AGN, which is roughly a factor of two larger than the positional uncertainty for all of our X-ray sources.        }
\centering

 \end{figure*}

\addtocounter{figure}{-1}


 \begin{figure*}
 \centering


\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{28_16550_-13_92369_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{28_28761_-13_96692_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{28_30403_-13_89717_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{29_99430_-8_82704_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{73_50511_2_96277_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{73_55489_2_95945_HubbleImage.jpg}



\caption{\label{XRaySourceImages}  Continued. The bottom right image in this panel is a galaxy with a previously unpublished partial Einstein ring.           }

 \end{figure*}


\addtocounter{figure}{-1}


 \begin{figure*}
 \centering


\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{139_43829_51_71885_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{146_80429_76_38735_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{151_72157_32_00314_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{177_39105_22_37405_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{181_55492_-8_79565_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{186_71535_21_87390_HubbleImage.jpg}


\caption{\label{XRaySourceImages}  Continued        }


 \end{figure*}

\addtocounter{figure}{-1}




 \begin{figure*}
 \centering


\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{186_75880_33_56825_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{212_63080_52_25929_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{224_31136_22_32598_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{243_90677_-6_18664_HubbleImage.jpg}
\includegraphics[width=0.37\textwidth,natwidth=541,natheight=579]{328_38098_17_69271_HubbleImage.jpg}



\caption{\label{XRaySourceImages}  Continued        }


 \end{figure*}

